Latent Noise Segmentation: How Neural Noise Leads to the Emergence of Segmentation and Grouping

Humans are able to segment images effortlessly without supervision using perceptual grouping. Here, we propose a counter-intuitive computational approach to solving unsupervised perceptual grouping and segmentation: that they arise because of neural noise, rather than in spite of it. We (1) mathematically demonstrate that under realistic assumptions, neural noise can be used to separate objects from each other; (2) that adding noise in a DNN enables the network to segment images even though it was never trained on any segmentation labels; and (3) that segmenting objects using noise results in segmentation performance that aligns with the perceptual grouping phenomena observed in humans, and is sample-efficient. We introduce the Good Gestalt (GG) datasets -- six datasets designed to specifically test perceptual grouping, and show that our DNN models reproduce many important phenomena in human perception, such as illusory contours, closure, continuity, proximity, and occlusion. Finally, we (4) show that our model improves performance on our GG datasets compared to other tested unsupervised models by $24.9\%$. Together, our results suggest a novel unsupervised segmentation method requiring few assumptions, a new explanation for the formation of perceptual grouping, and a novel potential benefit of neural noise.

==> AE_wrong_cluster_number.tex <==
\subsection{AEs, but not VAEs, Perceive the Wrong Number of Clusters}
\label{appendix:clustering}
In our Segmentation algorithm, the expected number of clusters is provided on an image-by-image basis as \textit{a priori} information for the model. 
In most cases, the expected number of clusters coincides with the actual clusters spontaneously formed by $\Delta \Tilde{\mathbf{X}}_i$, which can be qualitatively verified with a UMAP visualization \citep{mcinnes2018}.
However, there are exceptions where $\Delta \Tilde{\mathbf{X}}_i$ is not readily grouped into the expected numbers of clusters. 
We observe such exceptions in segmentation using AE on the GG Proximity dataset (when there only exists $1$ group of $6$ squares) and the GG Illusory Occlusion dataset. 
Here, we present the UMAP visualization for them using one example per dataset. 
Note that while not shown here, we observe that the qualitative pattern of the AE being unable to capture the expected number of clusters generally holds for these two cases.

In Figures ~\ref{fig: ae proximity umap} and ~\ref{fig: vae proximity umap}, we show the distribution of the vectors corresponding to each pixel in the $[C\times(N-1)]$-dimensional space where clustering is performed, when the models are confronted with an image from the GG Proximity dataset with $1$ group of $6$ squares.
The image and the expected target mask are shown in Figure~\ref{fig: ae proximity input target}.
In this case, the AE tends to separate the pixels belonging to the squares into $3$ clusters, perhaps as a result of being affected by training samples where there exist $3$ groups of $2$ squares; while the VAE tends to perceive the right number of clusters.
However, when given the expected number of clusters, which is $2$ in this case, the AE managed to nevertheless yield the correct segmentation mask (indicated by the inset in Figure~\ref{fig: ae proximity umap}).

\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.153\textwidth}
        \includegraphics[width=\textwidth]{figures/proximity_ae_wrong_cluster/orig.png}
        \caption{input (upper)\\target(lower)}
        \label{fig: ae proximity input target}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/proximity_ae_wrong_cluster/UMAP_AE.jpg}
        \caption{UMAP for AE}
        \label{fig: ae proximity umap}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/proximity_ae_wrong_cluster/UMAP_VAE.jpg}
        \caption{UMAP for VAE}
        \label{fig: vae proximity umap}
    \end{subfigure}
    \caption{The AE perceives the wrong numbers of clusters for the GG Proximity dataset with $1$ group of $6$ squares. (a) contains the input image and the expected mask. (b) and (c) show the visualization of $\Delta \Tilde{\mathbf{X}}^i$. Each dot corresponds to a pixel in the image. The visualization is made by using UMAP to reduce the $[C\times(N-1)]$-dimensional vector corresponding to each pixel to $2$ dimensions. 
    The color of the dots indicates which part the pixels correspond to. 
    The insets are the corresponding segmentation masks generated by the AE/VAE model.}
    \label{fig: ae proximity wrong cluster number}
\end{figure*}

A similar situation happens also for the GG Illusory Occlusion dataset. 
As shown in Figure~\ref{fig: ae illu_occlu wrong cluster number}, the AE tends to separate the background from the background stripes. 
We would expect these two parts to be grouped together, since they always co-vary with each other. 
Nonetheless, given the expected number of clusters, the AE manages to ultimately segment correctly.

\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.153\textwidth}
        \includegraphics[width=\textwidth]{figures/illusory_occl_ae_wrong_cluster/orig.png}
        \caption{input (upper)\\target(lower)}
        \label{fig: ae illu_occlu input target}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/illusory_occl_ae_wrong_cluster/UMAP_AE.jpg}
        \caption{UMAP for AE}
        \label{fig: ae illu_occlu umap}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/illusory_occl_ae_wrong_cluster/UMAP_VAE.jpg}
        \caption{UMAP for VAE}
        \label{fig: vae illu_occlu umap}
    \end{subfigure}
    \caption{The AE perceives the wrong number of clusters for the GG Illusory Occlusion Dataset. Please refer to the caption of Figure~\ref{fig: ae proximity wrong cluster number}.}
    \label{fig: ae illu_occlu wrong cluster number}
\end{figure*}






